Munchausen Iteration

We present a method for solving polynomial equations over idempotent omega-continuous semirings. The idea is to iterate over the semiring of functions rather than the semiring of interest, and only evaluate when needed. The key operation is substitution. In the initial step, we compute a linear completion of the system of equations that exhaustively inserts the equations into one another. With functions as approximants, the following steps insert the current approximant into itself. Since the iteration improves its precision by substitution rather than computation we named it Munchausen, after the fictional baron that pulled himself out of a swamp by his own hair. The first result shows that an evaluation of the n-th Munchausen approximant coincides with the 2^n-th Newton approximant. Second, we show how to compute linear completions with standard techniques from automata theory. In particular, we are not bound to (but can use) the notion of differentials prominent in Newton iteration.

==> commutative.tex <==
%!TEX root = main.tex
%
If multiplication in $\sr$ is commutative, the grammar construction can be simplified, and we gain a finite automaton describing the linear completion.
This yields a closed representation of the linear completion as a regular expression over $\vars \cup \sr$, on which further evaluation steps can be performed.
%
%Our main result shows that this sum can be represented as a regular language and, due to commutativity, even the Parikh image thereof.
%We then show that Newton iteration~\cite{EsparzaKieferLuttenberger2010} happens to compute precisely this regular language and thus the linear completion. 
%The difference with our approach is that Newton iteration is bound to computing derivatives and iterating matrices.
%Our result shows that (1) we are free in choosing the method of computation for the regular language and (2) we can work up to Parikh equivalence.
%This means we can apply all algorithms and tools that that have been developed for regular languages and semilinear sets. 
%In particular, we can apply minimization techniques to improve the performance of the following Munchausen iteration.
%Since the iteration will repeatedly apply the completion to itself, the size of the representation matters.
%
Since multiplication is commutative, we do not need to keep track of which occurrence of a variable is replaced, and we can always pull out the variable as a factor.
Equation~(\ref{Equation:DecompositionNonCommutative}) simplifies to
\begin{align}
    m = m^y \srmult y\ .\label{Equation:DecompositionCommutative}
\end{align}
Here, $m^y$ is the part that is not influenced by the following substitution $y\mapsto{m_{i_y}}$. 
Due to commutativity, $m^y$ is unique.

We define the automaton $A=(\vars\cup \set{\checkmark}, \set{\checkmark}, \Sigma, \bigcup_{y, z\in\vars}T_{y, z}\cup T )$.
It has as states the variables in the system of equations plus a distinguished accepting state $\checkmark$.
The letters $\Sigma = \vars\cup\sr$ are the variables and the semiring elements.
Actually, we will label transitions with words from $\Sigma^*$  and assume the automaton is extended with auxiliary states to turn them into single letters. 
The set of transitions $T_{y, z}$ contains for every monomial $m_{i_y}$ of $\vecat{f}{y}$ and every variable $z$ occurring in $m_{i_y}$ a transition from state $y$ to state $z$ labeled by $m_{i_y}^z$:
\begin{align*}
    T_{y, z} = \setcond{y \xrightarrow{\wordof{m_{i_y}^z}}z}{\vecat{f}{y}=\bigsradd_{i_y}m_{i_y}\text{ and }m_{i_y}= m_{i_y}^z \srmult z}\ .
\end{align*}
The remaining transitions add the missing variables, 
$T = \setcond{y\xrightarrow{y}\checkmark}{y\in\vars}$. 

We write $A_x$ for the automaton $A$ with initial state $x$. 
The first transitions from the initial state select the monomial of $\vecat{f}{x}$ to which the first linear monomial substitution is applied.
The second transition selects the monomial in $\vecat{f}{y}$ and so on. 
The final transition to the accepting state reflects the identity substitution (that forms the base case of a linear monomial substitution).


%
%Our main result shows that the language of this automaton is precisely the linear completion $\completionof{\vecat{f}{x}}$, when interpreting concatenation as multiplication in the semiring. 
%Since we work over a commutative io-semiring, having only the Parikh image is enough. 

\begin{proposition}
\label{Theorem:LinearCompletionCommutative}
    $\completionof{\vecat{f}{x}}
    = \srof{\langof{A_x}}
    %= \srof{\parikhof{\langof{A_x}}}
    $.
\end{proposition}
% -------------------------------------------------------------
% -------------------------------------------------------------
% -------------------------------------------------------------
% -------------------------------------------------------------
The first equality is by the discussion on the definition of the automaton, the second is immediate.

It is important to note that it is immediate to compute a Kleene polynomial (i.e. an expression involing $\sradd$, $\srmult$ and $\mbox{}^*$ over $\vars \cup \sr$ for $\srof{\langof{A_x}}$.
It is worth noting that the automata $A_x$ for the different variables $x$ only differ in their initial state, and hence share the transition monoid --- which may be helpful in algorithms.
Instead of computing a regular expression for each $x$ separately, it might be much more efficient to view the transitions of the automaton as a left-linear equation system and compute a regular expression for all $x$ simultaneously, i.e. by Tarjan's path-expression algorithm \cite{Tarjan}.
%
%We simply turn $A_x$ into a regular expression, replace concatenation by semiring multiplication, choice by semiring addition, and the Kleene star by the semiring Kleene star.
%Similarly, the Parikh image of a regular language is known to be a semilinear set.
%Turning this set into a Kleene polynomial is straightforward.
%Interestingly, we may also represent the set by an existential Presburger formula, using the flow equation. We return to this in Section~\ref{Section:Extension}.


==> extension.tex <==
%!TEX root = main.tex

\section{Extension}\label{Section:Extension}
\rfm{Can we reprove Verma, Seidl, Schwentick?}
The method can be generalized to polynomials that involve Kleene's star. 
Given a finite set of variables $\vars=\set{x_1,\ldots, x_k}$, we define the \emph{set of polynomials $\polysr$ over $\sr$} by
\begin{align*}
f\ ::=\ a\bnf x\bnf f\sradd g\bnf f\srmult g\bnf f^*\ . 
\end{align*}
Here, $a\in \sr$ and $x\in\vars$.


==> finitenoncommutative.tex <==
%
Assume $\sr$ is finite, meaning that its set of elements $S$ is finite. 
We consider equations over finitely many variables $\vars$.
Together, also the set of functions $\sr^\vars \to \sr$ is finite.
In this case, a Kleene iteration applied to the above linearized system of equations is sufficient to determine a closed form description of the linear completion.
In a second step, we insert the functions into one another.

\rfm{What is the convergence rate? We know the size of the domain of functions (relative to the sizes of $\sr$ and $\vars$).}

%
